On kinematical constraints in boson-boson systems

We consider the scattering of two-bosons with negative parity and spin 0 or 1. Starting from helicity partial-wave scattering amplitudes we derive transformations that eliminate all kinematical constraints. Such amplitudes are expected to satisfy partial-wave dispersion relations and therefore provide a suitable basis for data analysis and the construction of effective field theories. Our derivation relies on a decomposition of the various scattering amplitudes into suitable sets of invariant functions. A novel algebra was developed that permits the efficient computation of such functions in terms of computer algebra codes.

==> mybib.bib.tex <==
@Article{Stoica:2011cy,
     author    = "Stoica, S. and Lutz, M. F. M. and Scholten, O.",
     title     = "{On kinematical constraints in fermion-antifermion
                  systems}",
     journal   = "Phys. Rev. D, in print",
     year      = "2011",
     eprint    = "1106.5619",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     SLACcitation  = "%%CITATION = 1106.5619;%%"
}



@Article{Danilkin:2011fz,
     author    = "Danilkin, I. V. and Gil, L. I. R. and Lutz, M. F. M.",
     title     = "{Dynamical light vector mesons in low-energy scattering of
                  Goldstone bosons}",
     journal   = "Phys. Lett. B, in print",
     year      = "2011",
     eprint    = "1106.2230",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     SLACcitation  = "%%CITATION = 1106.2230;%%"
}


@Article{Nakanishi:1963zz,
     author    = "Nakanishi, Noboru",
     title     = "{Partial-Wave Bethe-Salpeter Equation}",
     journal   = "Phys. Rev.",
     volume    = "130",
     year      = "1963",
     pages     = "1230-1235",
     doi       = "10.1103/PhysRev.130.1230",
     SLACcitation  = "%%CITATION = PHRVA,130,1230;%%"
}

@Article{Berends:1967vi,
     author    = "Berends, Frits A. and Donnachie, A. and Weaver, D. L.",
     title     = "{Photoproduction and electroproduction of pions. 1.
                  Dispersion relation theory}",
     journal   = "Nucl. Phys.",
     volume    = "B4",
     year      = "1967",
     pages     = "1-53",
     doi       = "10.1016/0550-3213(67)90196-4",
     SLACcitation  = "%%CITATION = NUPHA,B4,1;%%"
}



@Article{Nieves:1998hp,
     author    = "Nieves, Juan and Ruiz Arriola, Enrique",
     title     = "{Bethe-Salpeter approach for meson meson scattering in
                  chiral  perturbation theory}",
     journal   = "Phys. Lett.",
     volume    = "B455",
     year      = "1999",
     pages     = "30-38",
     eprint    = "nucl-th/9807035",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-2693(99)00461-X",
     SLACcitation  = "%%CITATION = NUCL-TH/9807035;%%"
}

@Article{Nieves:1999bx,
     author    = "Nieves, Juan and Ruiz Arriola, Enrique",
     title     = "{Bethe-Salpeter approach for unitarized chiral perturbation
                  theory}",
     journal   = "Nucl. Phys.",
     volume    = "A679",
     year      = "2000",
     pages     = "57-117",
     eprint    = "hep-ph/9907469",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(00)00321-3",
     SLACcitation  = "%%CITATION = HEP-PH/9907469;%%"
}


@Article{Lutz:1999yr,
     author    = "Lutz, Matthias",
     title     = "{Effective chiral theory of nucleon nucleon scattering}",
     journal   = "Nucl. Phys.",
     volume    = "A677",
     year      = "2000",
     pages     = "241-312",
     eprint    = "nucl-th/9906028",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(00)00206-2",
     SLACcitation  = "%%CITATION = NUCL-TH/9906028;%%"
}



@Article{Lutz:2001mi,
     author    = "Lutz, M. F. M. and Wolf, G. and Friman, B.",
     title     = "{Scattering of vector mesons off nucleons}",
     journal   = "Nucl. Phys.",
     volume    = "A706",
     year      = "2002",
     pages     = "431-496",
     eprint    = "nucl-th/0112052",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.nuclphysa.2005.11.017",
     SLACcitation  = "%%CITATION = NUCL-TH/0112052;%%"
}




@Article{Lutz:2001dr,
     author    = "Lutz, M. F. M. and Kolomeitsev, E. E.",
     title     = "{Covariant meson baryon scattering with chiral and large
                  N(c)  constraints}",
     journal   = "Found. Phys.",
     volume    = "31",
     year      = "2001",
     pages     = "1671-1702",
     eprint    = "nucl-th/0105068",
     archivePrefix = "arXiv",
     doi       = "10.1023/A:1012655116247",
     SLACcitation  = "%%CITATION = NUCL-TH/0105068;%%"
}


@Article{Lutz:2001yb,
     author    = "Lutz, M. F. M. and Kolomeitsev, E. E.",
     title     = "{Relativistic chiral SU(3) symmetry, large N(c) sum rules
                  and meson  baryon scattering}",
     journal   = "Nucl. Phys.",
     volume    = "A700",
     year      = "2002",
     pages     = "193-308",
     eprint    = "nucl-th/0105042",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(01)01312-4",
     SLACcitation  = "%%CITATION = NUCL-TH/0105042;%%"
}

@article{Lutz:2003fm,
      author         = "Lutz, M.F.M. and Kolomeitsev, E.E.",
      title          = "{On meson resonances and chiral symmetry}",
      journal        = "Nucl.Phys.",
      volume         = "A730",
      pages          = "392-416",
      doi            = "10.1016/j.nuclphysa.2003.11.009",
      year           = "2004",
      eprint         = "nucl-th/0307039",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@Article{Gasparyan:2010xz,
     author    = "Gasparyan, A. and Lutz, M. F. M.",
     title     = "{Photon- and pion-nucleon interactions in a unitary and
                  causal effective field theory based on the chiral
                  Lagrangian}",
     journal   = "Nucl. Phys.",
     volume    = "A848",
     year      = "2010",
     pages     = "126-182",
     eprint    = "1003.3426",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1016/j.nuclphysa.2010.08.006",
     SLACcitation  = "%%CITATION = 1003.3426;%%"
}


@Article{Rarita:1941mf,
     author    = "Rarita, William and Schwinger, Julian",
     title     = "{On a theory of particles with half integral spin}",
     journal   = "Phys. Rev.",
     volume    = "60",
     year      = "1941",
     pages     = "61",
     doi       = "10.1103/PhysRev.60.61",
     SLACcitation  = "%%CITATION = PHRVA,60,61;%%"
}

@Article{Jacob:1959at,
     author    = "Jacob, M. and Wick, G. C.",
     title     = "{On the general theory of collisions for particles with
                  spin}",
     journal   = "Ann. Phys.",
     volume    = "7",
     year      = "1959",
     pages     = "404-428",
     doi       = "10.1016/0003-4916(59)90051-X",
     SLACcitation  = "%%CITATION = APNYA,7,404;%%"
}

@Article{Barut:1963zz,
     author    = "Barut, Asim O. and Muzinich, Ivan and Williams, David N.",
     title     = "{Construction of Invariant Scattering Amplitudes for
                  Arbitrary Spins and Analytic Continuation in Total Angular
                  Momentum}",
     journal   = "Phys. Rev.",
     volume    = "130",
     year      = "1963",
     pages     = "442-457",
     doi       = "10.1103/PhysRev.130.442",
     SLACcitation  = "%%CITATION = PHRVA,130,442;%%"
}

@article{CohenTannoudji:1968,
title = "Kinematical singularities, crossing matrix and kinematical constraints for two-body helicity amplitudes",
journal = "Annals of Physics",
volume = "46",
number = "2",
pages = "239 - 316",
year = "1968",
note = "",
issn = "0003-4916",
doi = "DOI: 10.1016/0003-4916(68)90243-1",
url = "http://www.sciencedirect.com/science/article/B6WB1-4DF52GS-1NW/2/f43af2dffa24a7e098fcfc0596291263",
author = "G. Cohen-Tannoudji and A. Morel and H. Navelet"
}

@Article{PhysRev.170.1606,
  title = {Threshold Kinematic Constraints and Correlations of Helicity Amplitudes},
  author = {Franklin, Jerrold },
  journal = {Phys. Rev.},
  volume = {170},
  number = {5},
  pages = {1606--1618},
  numpages = {12},
  year = {1968},
  month = {Jun},
  doi = {10.1103/PhysRev.170.1606},
  publisher = {American Physical Society}
}

@Article{PhysRev.142.1187,
  title = {General Method of Constructing Helicity Amplitudes Free from Kinematic Singularities and Zeros},
  author = {Wang, Ling-Lie Chau},
  journal = {Phys. Rev.},
  volume = {142},
  number = {4},
  pages = {1187--1194},
  numpages = {7},
  year = {1966},
  month = {Feb},
  doi = {10.1103/PhysRev.142.1187},
  publisher = {American Physical Society}
}

@Article{PhysRev.169.1248,
  title = {Kinematic Singularities and Threshold Relations for Helicity Amplitudes},
  author = {Jackson, J. D. and Hite, G. E.},
  journal = {Phys. Rev.},
  volume = {169},
  number = {5},
  pages = {1248--1274},
  numpages = {26},
  year = {1968},
  month = {May},
  doi = {10.1103/PhysRev.169.1248},
  publisher = {American Physical Society}
}

@Article{Scadron:1969rw,
     author    = "Scadron, M. D. and Jones, H. F.",
     title     = "{Covariant m functions for higher spin}",
     journal   = "Phys. Rev.",
     volume    = "173",
     year      = "1968",
     pages     = "1734-1744",
     doi       = "10.1103/PhysRev.173.1734",
     SLACcitation  = "%%CITATION = PHRVA,173,1734;%%"

@Article{Hara:1964zza,
     author    = "Hara, Yasuo",
     title     = "{Analyticity Properties of Helicity Amplitudes and
                  Construction of Kinematical Singularity-Free Amplitudes for
                  Any Spin}",
     journal   = "Phys. Rev.",
     volume    = "136",
     year      = "1964",
     pages     = "B507-B514",
     doi       = "10.1103/PhysRev.136.B507",
     SLACcitation  = "%%CITATION = PHRVA,136,B507;%%"
}

@Article{Chew:1957tf,
     author    = "Chew, G. F. and Goldberger, M. L. and Low, F. E. and Nambu,
                  Yoichiro",
     title     = "{Relativistic dispersion relation approach to photomeson
                  production}",
     journal   = "Phys. Rev.",
     volume    = "106",
     year      = "1957",
     pages     = "1345-1355",
     doi       = "10.1103/PhysRev.106.1345",
     SLACcitation  = "%%CITATION = PHRVA,106,1345;%%"
}

@Article{Lutz:2003jw,
     author    = "Lutz, M. F. M. and Kolomeitsev, E. E.",
     title     = "{On charm baryon resonances and chiral symmetry}",
     journal   = "Nucl. Phys.",
     volume    = "A730",
     year      = "2004",
     pages     = "110-120",
     eprint    = "hep-ph/0307233",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.nuclphysa.2003.10.012",
     SLACcitation  = "%%CITATION = HEP-PH/0307233;%%"
}
@Article{Bardeen:1969aw,
     author    = "Bardeen, William A. and Tung, W. K.",
     title     = "{Invariant amplitudes for photon processes}",
     journal   = "Phys. Rev.",
     volume    = "173",
     year      = "1968",
     pages     = "1423-1433",
     doi       = "10.1103/PhysRev.173.1423",
     SLACcitation  = "%%CITATION = PHRVA,173,1423;%%"
}

@Article{Ball:1961zza,
     author    = "Ball, James Stutsman",
     title     = "{Application of the Mandelstam Representation to
                  Photoproduction of Pions from Nucleons}",
     journal   = "Phys. Rev.",
     volume    = "124",
     year      = "1961",
     pages     = "2014-2028",
     doi       = "10.1103/PhysRev.124.2014",
     SLACcitation  = "%%CITATION = PHRVA,124,2014;%%"
}

@Article{Nakanishi:1962,
  title = {Proof of Partial-Wave Dispersion Relations in Perturbation Theory},
  author = {Nakanishi, Noboru },
  journal = {Phys. Rev.},
  volume = {126},
  number = {3},
  pages = {1225--1226},
  numpages = {1},
  year = {1962},
  month = {May},
  doi = {10.1103/PhysRev.126.1225},
  publisher = {American Physical Society}
}

@Article{Berends:1967vi,
     author    = "Berends, Frits A. and Donnachie, A. and Weaver, D. L.",
     title     = "{Photoproduction and electroproduction of pions. 1.
                  Dispersion relation theory}",
     journal   = "Nucl. Phys.",
     volume    = "B4",
     year      = "1967",
     pages     = "1-53",
     doi       = "10.1016/0550-3213(67)90196-4",
     SLACcitation  = "%%CITATION = NUPHA,B4,1;%%"
}


@Article{Mandelstam:1958xc,
     author    = "Mandelstam, S.",
     title     = "{Determination of the pion - nucleon scattering amplitude
                  from dispersion relations and unitarity. General theory}",
     journal   = "Phys. Rev.",
     volume    = "112",
     year      = "1958",
     pages     = "1344-1360",
     doi       = "10.1103/PhysRev.112.1344",
     SLACcitation  = "%%CITATION = PHRVA,112,1344;%%"
}

@Thesis{Williams:1963,
   author = {D.N.~ Williams}
   title = {Construction of Invariant Scalar Amplitudes without Kinematical Singularities
            for Arbitrary-Spin Nonzero-Mass Two-Body Scattering Processes}
   publisher = {Lawrence Radiation Laboratory, University of California, Berkeley}
}


@Article{MAMIA2-11/09,
     author    = "{The A2 Collaboration}",
     title     = "{Measurement of the Proton Spin Polarizabilities}",
     journal   = "Exp.-Nr. A2-11/09",
     volume    = "",
     year      = "",
     pages     = "",
     eprint    = "",
     archivePrefix = "",
     doi       = "",
     SLACcitation  = "%%CITATION = NUCL-TH/0403088;%%"
}

@Article{Weller:2009zza,
     author    = "Weller, Henry R. and others",
     title     = "{Research opportunities at the upgraded HIgammaS
                  facility}",
     journal   = "Prog. Part. Nucl. Phys.",
     volume    = "62",
     year      = "2009",
     pages     = "257-303",
     doi       = "10.1016/j.ppnp.2008.07.001",
     SLACcitation  = "%%CITATION = PPNPD,62,257;%%"
}


@Article{Beane:2004ra,
     author    = "Beane, S. R. and Malheiro, M. and McGovern, J. A. and
                  Phillips, Daniel R. and van Kolck, U.",
     title     = "{Compton scattering on the proton, neutron, and deuteron in
                  chiral perturbation theory to O($Q^4$)}",
     journal   = "Nucl. Phys.",
     volume    = "A747",
     year      = "2005",
     pages     = "311-361",
     eprint    = "nucl-th/0403088",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.nuclphysa.2004.09.068",
     SLACcitation  = "%%CITATION = NUCL-TH/0403088;%%"
}

@Article{Pascalutsa:2005vq,
     author    = "Pascalutsa, Vladimir and Vanderhaeghen, Marc",
     title     = "{Chiral effective-field theory in the Delta(1232) region.
                  I: Pion  electroproduction on the nucleon}",
     journal   = "Phys. Rev.",
     volume    = "D73",
     year      = "2006",
     pages     = "034003",
     eprint    = "hep-ph/0512244",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevD.73.034003",
     SLACcitation  = "%%CITATION = HEP-PH/0512244;%%"
}

@Article{Weinberg:1990rz,
     author    = "Weinberg, Steven",
     title     = "{Nuclear forces from chiral Lagrangians}",
     journal   = "Phys. Lett.",
     volume    = "B251",
     year      = "1990",
     pages     = "288-292",
     doi       = "10.1016/0370-2693(90)90938-3",
     SLACcitation  = "%%CITATION = PHLTA,B251,288;%%"
}

@Article{Weinberg:1991um,
     author    = "Weinberg, Steven",
     title     = "{Effective chiral Lagrangians for nucleon - pion
                  interactions and nuclear forces}",
     journal   = "Nucl. Phys.",
     volume    = "B363",
     year      = "1991",
     pages     = "3-18",
     doi       = "10.1016/0550-3213(91)90231-L",
     SLACcitation  = "%%CITATION = NUPHA,B363,3;%%"
}


@Article{Pascalutsa:2002pi,
     author    = "Pascalutsa, Vladimir and Phillips, Daniel R.",
     title     = "{Effective theory of the Delta(1232) in Compton scattering
                  off the nucleon}",
     journal   = "Phys. Rev.",
     volume    = "C67",
     year      = "2003",
     pages     = "055202",
     eprint    = "nucl-th/0212024",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.67.055202",
     SLACcitation  = "%%CITATION = NUCL-TH/0212024;%%"
}


@Article{Pascalutsa:2007yg,
     author    = "Pascalutsa, Vladimir",
     title     = "{The Delta(1232) Resonance in Chiral Effective Field
                  Theory}",
     journal   = "Prog. Part. Nucl. Phys.",
     volume    = "61",
     year      = "2008",
     pages     = "27-33",
     eprint    = "0712.3919",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1016/j.ppnp.2007.12.023",
     SLACcitation  = "%%CITATION = 0712.3919;%%"
}

@Article{Long:2009wq,
     author    = "Long, Bingwei and van Kolck, U.",
     title     = "{$\pi N$ Scattering in the $\Delta(1232)$ Region in an
                  Effective Field Theory}",
     journal   = "Nucl. Phys.",
     volume    = "A840",
     year      = "2010",
     pages     = "39-75",
     eprint    = "0907.4569",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     SLACcitation  = "%%CITATION = 0907.4569;%%"
}

@Article{Datta:1996jb,
     author    = "Datta, Alakabha and Pakvasa, Sandip",
     title     = "{Pion nucleon phase shifts in heavy baryon chiral
                  perturbation theory}",
     journal   = "Phys. Rev.",
     volume    = "D56",
     year      = "1997",
     pages     = "4322-4327",
     eprint    = "hep-ph/9606277",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevD.56.4322",
     SLACcitation  = "%%CITATION = HEP-PH/9606277;%%"
}

@Article{Fettes:2000bb,
     author    = "Fettes, Nadia and Meissner, Ulf G.",
     title     = "{Pion nucleon scattering in an effective chiral field
                  theory with  explicit spin-3/2 fields}",
     journal   = "Nucl. Phys.",
     volume    = "A679",
     year      = "2001",
     pages     = "629-670",
     eprint    = "hep-ph/0006299",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(00)00368-7",
     SLACcitation  = "%%CITATION = HEP-PH/0006299;%%"
}

@Article{Ellis:1997kc,
     author    = "Ellis, Paul J. and Tang, Hua-Bin",
     title     = "{Pion nucleon scattering in a new approach to chiral
                  perturbation  theory}",
     journal   = "Phys. Rev.",
     volume    = "C57",
     year      = "1998",
     pages     = "3356-3375",
     eprint    = "hep-ph/9709354",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.57.3356",
     SLACcitation  = "%%CITATION = HEP-PH/9709354;%%"
}


@Article{Torikoshi:2002bt,
     author    = "Torikoshi, Kenichi and Ellis, Paul J.",
     title     = "{Low energy pion nucleon scattering in the heavy baryon and
                  infrared schemes}",
     journal   = "Phys. Rev.",
     volume    = "C67",
     year      = "2003",
     pages     = "015208",
     eprint    = "nucl-th/0208049",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.67.015208",
     SLACcitation  = "%%CITATION = NUCL-TH/0208049;%%"
}


@Article{Bernard:2007zu,
     author    = "Bernard, Veronique",
     title     = "{Chiral Perturbation Theory and Baryon Properties}",
     journal   = "Prog. Part. Nucl. Phys.",
     volume    = "60",
     year      = "2008",
     pages     = "82-160",
     eprint    = "0706.0312",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1016/j.ppnp.2007.07.001",
     SLACcitation  = "%%CITATION = 0706.0312;%%"
}
@Article{Bardeen:1969aw,
     author    = "Bardeen, William A. and Tung, W. K.",
     title     = "{Invariant amplitudes for photon processes}",
     journal   = "Phys. Rev.",
     volume    = "173",
     year      = "1968",
     pages     = "1423-1433",
     doi       = "10.1103/PhysRev.173.1423",
     SLACcitation  = "%%CITATION = PHRVA,173,1423;%%"
}
@Article{MacDowell:1959zza,
     author    = "MacDowell, S. W.",
     title     = "{Analytic Properties of Partial Amplitudes in Meson-Nucleon
                  Scattering}",
     journal   = "Phys. Rev.",
     volume    = "116",
     year      = "1959",
     pages     = "774-778",
     doi       = "10.1103/PhysRev.116.774",
     SLACcitation  = "%%CITATION = PHRVA,116,774;%%"
}
@Article{Chew:1957tf,
     author    = "Chew, G. F. and Goldberger, M. L. and Low, F. E. and Nambu,
                  Yoichiro",
     title     = "{Relativistic dispersion relation approach to photomeson
                  production}",
     journal   = "Phys. Rev.",
     volume    = "106",
     year      = "1957",
     pages     = "1345-1355",
     doi       = "10.1103/PhysRev.106.1345",
     SLACcitation  = "%%CITATION = PHRVA,106,1345;%%"
}
@Article{Mandelstam:1958xc,
     author    = "Mandelstam, S.",
     title     = "{Determination of the pion - nucleon scattering amplitude
                  from dispersion relations and unitarity. General theory}",
     journal   = "Phys. Rev.",
     volume    = "112",
     year      = "1958",
     pages     = "1344-1360",
     doi       = "10.1103/PhysRev.112.1344",
     SLACcitation  = "%%CITATION = PHRVA,112,1344;%%"
}
@Article{Ciulli:1973iv,
     author    = "Ciulli, S. and Pomponiu, C. and Sabba-Stefanescu, I. and
                  Steinbrecher, G.",
     title     = "{CDD POLES, INELASTICITIES AND OPTIMIZATION OF N/D
                  EQUATIONS}",
     journal   = "Nucl. Phys.",
     volume    = "B71",
     year      = "1974",
     pages     = "269",
     doi       = "10.1016/0550-3213(74)90396-4",
     SLACcitation  = "%%CITATION = NUPHA,B71,269;%%"
}
@Article{Ball:1961zza,
     author    = "Ball, James Stutsman",
     title     = "{Application of the Mandelstam Representation to
                  Photoproduction of Pions from Nucleons}",
     journal   = "Phys. Rev.",
     volume    = "124",
     year      = "1961",
     pages     = "2014-2028",
     doi       = "10.1103/PhysRev.124.2014",
     SLACcitation  = "%%CITATION = PHRVA,124,2014;%%"
}


@Article{Hornidge2003,
     author    = "Hornidge, D.",
     title     = "{Proposal for an experiment}",
     journal   = "MAMI-A2/6-03",
     volume    = "",
     year      = "",
     pages     = "",
     eprint    = "",
     archivePrefix = "",
     doi       = "",
     SLACcitation  = ""
}

@Article{Bernstein2009,
     author    = "Berstein, A.",
     title     = "{Proposal for an experiment}",
     journal   = "MAMI-A2/10-09",
     volume    = "",
     year      = "",
     pages     = "",
     eprint    = "",
     archivePrefix = "",
     doi       = "",
     SLACcitation  = ""
}

@Article{Schumacher:2005an,
     author    = "Schumacher, Martin",
     title     = "{Polarizability of the Nucleon and Compton Scattering}",
     journal   = "Prog. Part. Nucl. Phys.",
     volume    = "55",
     year      = "2005",
     pages     = "567-646",
     eprint    = "hep-ph/0501167",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.ppnp.2005.01.033",
     SLACcitation  = "%%CITATION = HEP-PH/0501167;%%"
}

@Article{L'vov:1996xd,
     author    = "L'vov, A. I. and Petrun'kin, V. A. and Schumacher, M.",
     title     = "{Dispersion theory of proton Compton scattering in the
                  first and second resonance regions}",
     journal   = "Phys. Rev.",
     volume    = "C55",
     year      = "1997",
     pages     = "359-377",
     doi       = "10.1103/PhysRevC.55.359",
     SLACcitation  = "%%CITATION = PHRVA,C55,359;%%"
}
@Article{Babusci:1998ww,
     author    = "Babusci, D. and Giordano, G. and L'vov, A. I. and Matone,
                  G. and Nathan, A. M.",
     title     = "{Low-energy Compton scattering of polarized photons on
                  polarized  nucleons}",
     journal   = "Phys. Rev.",
     volume    = "C58",
     year      = "1998",
     pages     = "1013-1041",
     eprint    = "hep-ph/9803347",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.58.1013",
     SLACcitation  = "%%CITATION = HEP-PH/9803347;%%"
}
@Article{Bernard:1995cj,
     author    = "Bernard, V. and Kaiser, Norbert and Meissner, Ulf-G.",
     title     = "{Chiral symmetry and the reaction $\gamma p \to \pi~0 p$}",
     journal   = "Phys. Lett.",
     volume    = "B378",
     year      = "1996",
     pages     = "337-341",
     eprint    = "hep-ph/9512234",
     archivePrefix = "arXiv",
     doi       = "10.1016/0370-2693(96)00356-5",
     SLACcitation  = "%%CITATION = HEP-PH/9512234;%%"
}

@Article{Bernard:1996ti,
     author    = "Bernard, V. and Kaiser, Norbert and Meissner, Ulf-G.",
     title     = "{Chiral corrections to the Kroll-Ruderman theorem}",
     journal   = "Phys. Lett.",
     volume    = "B383",
     year      = "1996",
     pages     = "116-120",
     eprint    = "hep-ph/9603278",
     archivePrefix = "arXiv",
     doi       = "10.1016/0370-2693(96)00699-5",
     SLACcitation  = "%%CITATION = HEP-PH/9603278;%%"
}


@Article{Bernard:2001gz,
     author    = "Bernard, Veronique and Kaiser, Norbert and Meissner, Ulf-G.
                  ",
     title     = "{Aspects of near threshold neutral pion photoproduction off
                  protons}",
     journal   = "Eur. Phys. J.",
     volume    = "A11",
     year      = "2001",
     pages     = "209-216",
     eprint    = "hep-ph/0102066",
     archivePrefix = "arXiv",
     doi       = "10.1007/s100500170085",
     SLACcitation  = "%%CITATION = HEP-PH/0102066;%%"
}


@Article{Schmidt:2001vg,
     author    = "Schmidt, A. and others",
     title     = "{Test of low-energy theorems for p(gamma(pol.),pi0)p in the
                  threshold  region}",
     journal   = "Phys. Rev. Lett.",
     volume    = "87",
     year      = "2001",
     pages     = "232501",
     eprint    = "nucl-ex/0105010",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevLett.87.232501",
     SLACcitation  = "%%CITATION = NUCL-EX/0105010;%%"
}


@Article{Donnachie:1966,
     author    = "Donnachie, A. and Shaw, G.",
     title     = "{Photopion Production, Disperions Relations, and gamma-rho-pi Coupling}",
     journal   = "Ann. Phys.",
     volume    = "37",
     year      = "1966",
     pages     = "333-364",
     doi       = "",
     SLACcitation  = "%%%%"
}

@Article{Walker:1968xu,
     author    = "Walker, R. L.",
     title     = "{Phenomenological analysis of single pion
                  photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "182",
     year      = "1969",
     pages     = "1729-1748",
     doi       = "10.1103/PhysRev.182.1729",
     SLACcitation  = "%%CITATION = PHRVA,182,1729;%%"
}
@Article{Chen:1972rq,
     author    = "Chen, Chih Kwan",
     title     = "{Generalized partial-wave dispersion relation and the n/d
                  method}",
     journal   = "Phys. Rev.",
     volume    = "D5",
     year      = "1972",
     pages     = "1464-1471",
     doi       = "10.1103/PhysRevD.5.1464",
     SLACcitation  = "%%CITATION = PHRVA,D5,1464;%%"
}
@Article{Johnson:1979jy,
     author    = "Johnson, Porter W. and Warnock, Robert Lee",
     title     = "{Solution of the unitarity equation with overlapping left
                  and right cuts: a tool for study of the s* and similar
                  systems}",
     journal   = "J. Math. Phys.",
     volume    = "22",
     year      = "1981",
     pages     = "385",
     doi       = "10.1063/1.524904",
     SLACcitation  = "%%CITATION = JMAPA,22,385;%%"
}
@Article{Sommer:1970mr,
     author    = "Sommer, G.",
     title     = "{Present state of rigorous analytic properties of
                  scattering amplitudes}",
     journal   = "Fortsch. Phys.",
     volume    = "18",
     year      = "1970",
     pages     = "577-688",
     doi       = "10.1002/prop.19700181102",
     SLACcitation  = "%%CITATION = FPYKA,18,577;%%"
}
@Article{Castillejo:1955ed,
     author    = "Castillejo, L. and Dalitz, R. H. and Dyson, F. J.",
     title     = "{Low's scattering equation for the charged and neutral
                  scalar theories}",
     journal   = "Phys. Rev.",
     volume    = "101",
     year      = "1956",
     pages     = "453-458",
     doi       = "10.1103/PhysRev.101.453",
     SLACcitation  = "%%CITATION = PHRVA,101,453;%%"
}
@Article{Mandelstam:1963,
     author    = "Mandelstam, S.",
     title     = "{Regge poles as consequences of analyticity and unitarity}",
     journal   = "Annals Phys.",
     volume    = "21",
     year      = "1963",
     pages     = "302-343"
}
@Article{Frazer:1961zz,
     author    = "Frazer, William R.",
     title     = "{Applications of Conformal Mapping to the Phenomenological
                  Representation of Scattering Amplitudes}",
     journal   = "Phys. Rev.",
     volume    = "123",
     year      = "1961",
     pages     = "2180-2182",
     doi       = "10.1103/PhysRev.123.2180",
     SLACcitation  = "%%CITATION = PHRVA,123,2180;%%"
}
@book{Collins:1968,
  author = "{P.~D.~B.~Collins and E.~J.~Squires}",
  title = "{Regge Poles in Particle Physics}",
  year = 1968,
  publisher = "{Julius Springer-Verlag}",
  address = "{Berlin}"
}

@Article{Scholten:1996mw,
     author    = "Scholten, O. and Korchin, A. Yu. and Pascalutsa, V. and Van
                  Neck, D.",
     title     = "{Pion and photon induced reactions on the nucleon in a
                  unitary model}",
     journal   = "Phys. Lett.",
     volume    = "B384",
     year      = "1996",
     pages     = "13-19",
     eprint    = "nucl-th/9604014",
     archivePrefix = "arXiv",
     doi       = "10.1016/0370-2693(96)00825-8",
     SLACcitation  = "%%CITATION = NUCL-TH/9604014;%%"
}
@Article{Shklyar:2004ba,
     author    = "Shklyar, V. and Lenske, H. and Mosel, U. and Penner, G.",
     title     = "{Coupled-channel analysis of the omega-meson production in
                  pi N and  gamma N reactions for cm energies up to 2-GeV}",
     journal   = "Phys. Rev.",
     volume    = "C71",
     year      = "2005",
     pages     = "055206",
     eprint    = "nucl-th/0412029",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.71.055206",
     SLACcitation  = "%%CITATION = NUCL-TH/0412029;%%"
}
@Article{Penner:2002md,
     author    = "Penner, G. and Mosel, U.",
     title     = "{Vector meson production and nucleon resonance analysis in
                  a coupled-channel approach for energies $m_N < sqrt(s) < 2$
                  GeV II: photon-induced results}",
     journal   = "Phys. Rev.",
     volume    = "C66",
     year      = "2002",
     pages     = "055212",
     eprint    = "nucl-th/0207069",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.66.055212",
     SLACcitation  = "%%CITATION = NUCL-TH/0207069;%%"
}
@Article{Pascalutsa:2006up,
     author    = "Pascalutsa, Vladimir and Vanderhaeghen, Marc and Yang, Shin
                  Nan",
     title     = "{Electromagnetic excitation of the Delta(1232)-resonance}",
     journal   = "Phys. Rept.",
     volume    = "437",
     year      = "2007",
     pages     = "125-232",
     eprint    = "hep-ph/0609004",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.physrep.2006.09.006",
     SLACcitation  = "%%CITATION = HEP-PH/0609004;%%"
}
@Article{Matsuyama:2006rp,
     author    = "Matsuyama, A. and Sato, T. and Lee, T. -S. H.",
     title     = "{Dynamical coupled-channel model of meson production
                  reactions in the nucleon resonance region}",
     journal   = "Phys. Rept.",
     volume    = "439",
     year      = "2007",
     pages     = "193-253",
     eprint    = "nucl-th/0608051",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.physrep.2006.12.003",
     SLACcitation  = "%%CITATION = NUCL-TH/0608051;%%"
}

@Article{PhysRev.130.478,
title = {Analysis of Partial-Wave Dispersion Relations},
author = {Frye, Graham  and Warnock, Robert Lee},
journal = {Phys. Rev.},
volume = {130},
number = {1},
pages = {478--494},
numpages = {16},
year = {1963},
month = {Apr},
doi = {10.1103/PhysRev.130.478},
publisher = {American Physical Society}
}

@Article{Chew:1960iv,
author    = "Chew, Geoffrey F. and Mandelstam, Stanley",
title     = "{Theory of low-energy pion pion interactions}",
journal   = "Phys. Rev.",
volume    = "119",
year      = "1960",
pages     = "467-477",
doi       = "10.1103/PhysRev.119.467",
SLACcitation  = "%%CITATION = PHRVA,119,467;%%"
}

@Article{Lutz:Kolomeitsev:2010,
     author    = "Lutz, M. F. M.  and  Kolomeitsev, E. E.",
     title     = "{Baryon resonances in the hadrogenesis conjecture}",
     journal   = "in preparation",
     volume    = "",
     year      = "2010",
     pages     = "",
     eprint    = "in preparation",
     archivePrefix = "arXiv"
}
@Article{Lutz:2001yb,
     author    = "Lutz, M. F. M. and Kolomeitsev, E. E.",
     title     = "{Relativistic chiral SU(3) symmetry, large N(c) sum rules
                  and meson  baryon scattering}",
     journal   = "Nucl. Phys.",
     volume    = "A700",
     year      = "2002",
     pages     = "193-308",
     eprint    = "nucl-th/0105042",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(01)01312-4",
     SLACcitation  = "%%CITATION = NUCL-TH/0105042;%%"
}
@Article{Zachariasen:1961,
  title = {Relativistic Model Field Theory with Finite Self-Masses},
  author = {Zachariasen, F. },
  journal = {Phys. Rev.},
  volume = {121},
  number = {6},
  pages = {1851--1862},
  numpages = {11},
  year = {1961},
  month = {Mar},
  doi = {10.1103/PhysRev.121.1851},
  publisher = {American Physical Society}
}
@Article{Koch:1985bn,
     author    = "Koch, R.",
     title     = "{A Calculation of Low-Energy pi N Partial Waves Based on
                  Fixed t Analyticity}",
     journal   = "Nucl. Phys.",
     volume    = "A448",
     year      = "1986",
     pages     = "707",
     doi       = "10.1016/0375-9474(86)90438-0",
     SLACcitation  = "%%CITATION = NUPHA,A448,707;%%"
}
@Article{Arndt:2006bf,
     author    = "Arndt, R. A. and Briscoe, W. J. and Strakovsky, I. I. and
                  Workman, R. L.",
     title     = "{Extended Partial-Wave Analysis of piN Scattering Data}",
     journal   = "Phys. Rev.",
     volume    = "C74",
     year      = "2006",
     pages     = "045205",
     eprint    = "nucl-th/0605082",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.74.045205",
     SLACcitation  = "%%CITATION = NUCL-TH/0605082;%%"
}
@Article{Drechsel:2007if,
     author    = "Drechsel, D. and Kamalov, S. S. and Tiator, L.",
     title     = "{Unitary Isobar Model - MAID2007}",
     journal   = "Eur. Phys. J.",
     volume    = "A34",
     year      = "2007",
     pages     = "69-97",
     eprint    = "0710.0306",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1140/epja/i2007-10490-6",
     SLACcitation  = "%%CITATION = 0710.0306;%%"
}
@Article{Arndt:2002xv,
     author    = "Arndt, R. A. and Briscoe, W. J. and Strakovsky, I. I. and
                  Workman, R. L.",
     title     = "{Analysis of Pion Photoproduction Data}",
     journal   = "Phys. Rev.",
     volume    = "C66",
     year      = "2002",
     pages     = "055213",
     eprint    = "nucl-th/0205067",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.66.055213",
     SLACcitation  = "%%CITATION = NUCL-TH/0205067;%%"
}
@Article{Fettes:1998ud,
     author    = "Fettes, Nadia and Meissner, Ulf-G. and Steininger, Sven",
     title     = "{Pion nucleon scattering in chiral perturbation theory.  I:
                  Isospin-symmetric case}",
     journal   = "Nucl. Phys.",
     volume    = "A640",
     year      = "1998",
     pages     = "199-234",
     eprint    = "hep-ph/9803266",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(98)00452-7",
     SLACcitation  = "%%CITATION = HEP-PH/9803266;%%"
}
@Article{Bart:1969ue,
     author    = "Bart, G. R. and Warnock, R. L.",
     title     = "{Empirical n/d potential and castillejo-dalitz-dyson poles
                  in the pion-nucleon p(11) state}",
     journal   = "Phys. Rev. Lett.",
     volume    = "22",
     year      = "1969",
     pages     = "1081-1084",
     doi       = "10.1103/PhysRevLett.22.1081",
     SLACcitation  = "%%CITATION = PRLTA,22,1081;%%"
}
@Article{Korkmaz:1999sg,
     author    = "Korkmaz, E. and others",
     title     = "{Measurement of the gamma p --> pi+ n reaction near
                  threshold}",
     journal   = "Phys. Rev. Lett.",
     volume    = "83",
     year      = "1999",
     pages     = "3609-3612",
     doi       = "10.1103/PhysRevLett.83.3609",
     SLACcitation  = "%%CITATION = PRLTA,83,3609;%%"
}
@Article{Kovash:1997tj,
     author    = "Kovash, M. A.",
 collaboration = "E643",
     title     = "{Total cross-sections for pi- p $\to$ gamma n at 10-MeV to
                  20-MeV}",
     journal   = "PiN Newslett.",
     volume    = "12N3",
     year      = "1997",
     pages     = "51-55",
     SLACcitation  = "%%CITATION = 00076,12N3,51;%%"
}
@Article{Fuchs:1996ja,
     author    = "Fuchs, M. and others",
     title     = "{Neutral pion photoproduction from the proton near
                  threshold}",
     journal   = "Phys. Lett.",
     volume    = "B368",
     year      = "1996",
     pages     = "20-25",
     doi       = "10.1016/0370-2693(95)01488-8",
     SLACcitation  = "%%CITATION = PHLTA,B368,20;%%"
}
@Article{Bergstrom:1996fq,
     author    = "Bergstrom, J. C. and others",
     title     = "{Measurement of the H-1 (gamma, pi0) cross-section near
                  threshold}",
     journal   = "Phys. Rev.",
     volume    = "C53",
     year      = "1996",
     pages     = "1052-1056",
     doi       = "10.1103/PhysRevC.53.R1052",
     SLACcitation  = "%%CITATION = PHRVA,C53,1052;%%"
}

@Article{Hanstein:1996bd,
     author    = "Hanstein, O. and Drechsel, D. and Tiator, L.",
     title     = "{A dispersion theoretical approach to the threshold
                  amplitudes of pion  photoproduction}",
     journal   = "Phys. Lett.",
     volume    = "B399",
     year      = "1997",
     pages     = "13-21",
     eprint    = "nucl-th/9612057",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-2693(97)00272-4",
     SLACcitation  = "%%CITATION = NUCL-TH/9612057;%%"
}



@Article{Procura:2006bj,
     author    = "Procura, M. and Musch, B. U. and Wollenweber, T. and
                  Hemmert, T. R. and Weise, W.",
     title     = "{Nucleon mass: From lattice QCD to the chiral limit}",
     journal   = "Phys. Rev.",
     volume    = "D73",
     year      = "2006",
     pages     = "114510",
     eprint    = "hep-lat/0603001",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevD.73.114510",
     SLACcitation  = "%%CITATION = HEP-LAT/0603001;%%"
}


@Article{Bergstrom:1997jc,
     author    = "Bergstrom, J. C. and Igarashi, R. and Vogt, J. M.",
     title     = "{Measurement of the H-1(gamma,pi0) cross-section near
                  threshold. II: Pion angular distributions}",
     journal   = "Phys. Rev.",
     volume    = "C55",
     year      = "1997",
     pages     = "2016-2023",
     doi       = "10.1103/PhysRevC.55.2016",
     SLACcitation  = "%%CITATION = PHRVA,C55,2016;%%"
}



@Article{Schmidt:2001,
     author    = "Schmidt, Axel",
     journal   = "PhD thesis, Mainz (2001),  http://wwwa2.kph.uni-maiz.de/A2/",
     year      = "2001"
}

@Article{Bernard:1992nc,
     author    = "Bernard, Veronique and Kaiser, Norbert and Meissner, Ulf G.
                  ",
     title     = "{Threshold pion photoproduction in chiral perturbation
                  theory}",
     journal   = "Nucl. Phys.",
     volume    = "B383",
     year      = "1992",
     pages     = "442-496",
     doi       = "10.1016/0550-3213(92)90085-P",
     SLACcitation  = "%%CITATION = NUPHA,B383,442;%%"
}
@Article{Gasparyan:2003fp,
     author    = "Gasparyan, A. M. and Haidenbauer, J. and Hanhart, C. and
                  Speth, J.",
     title     = "{Pion nucleon scattering in a meson exchange model}",
     journal   = "Phys. Rev.",
     volume    = "C68",
     year      = "2003",
     pages     = "045207",
     eprint    = "nucl-th/0307072",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.68.045207",
     SLACcitation  = "%%CITATION = NUCL-TH/0307072;%%"
}
@Article{Krehl:1999km,
     author    = "Krehl, O. and Hanhart, C. and Krewald, S. and Speth, J.",
     title     = "{What is the structure of the Roper resonance?}",
     journal   = "Phys. Rev.",
     volume    = "C62",
     year      = "2000",
     pages     = "025207",
     eprint    = "nucl-th/9911080",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.62.025207",
     SLACcitation  = "%%CITATION = NUCL-TH/9911080;%%"
}
@Article{Bernard:1995dp,
     author    = "Bernard, V. and Kaiser, Norbert and Meissner, Ulf-G.",
     title     = "{Chiral dynamics in nucleons and nuclei}",
     journal   = "Int. J. Mod. Phys.",
     volume    = "E4",
     year      = "1995",
     pages     = "193-346",
     eprint    = "hep-ph/9501384",
     archivePrefix = "arXiv",
     doi       = "10.1142/S0218301395000092",
     SLACcitation  = "%%CITATION = HEP-PH/9501384;%%"
}
@Article{Blanpied:2001ae,
     author    = "Blanpied, G. and others",
     title     = "{$N \to \Delta$ transition and proton polarizabilities from
                  measurements of $p$( $\gamma$ polarized , $\gamma$ ),
                 $p$($\gamma$ polarized , $\pi^0$), and $p$( $\gamma$ polarized , $\pi^+$)}",
     journal   = "Phys. Rev.",
     volume    = "C64",
     year      = "2001",
     pages     = "025203",
     doi       = "10.1103/PhysRevC.64.025203",
     SLACcitation  = "%%CITATION = PHRVA,C64,025203;%%"
}
@Article{Hallin:1993ft,
     author    = "Hallin, E. L. and others",
     title     = "{Compton scattering from the proton}",
     journal   = "Phys. Rev.",
     volume    = "C48",
     year      = "1993",
     pages     = "1497-1507",
     doi       = "10.1103/PhysRevC.48.1497",
     SLACcitation  = "%%CITATION = PHRVA,C48,1497;%%"
}
@Article{OlmosdeLeon:2001zn,
     author    = "Olmos de Leon, V. and others",
     title     = "{Low-energy Compton scattering and the polarizabilities of
                  the proton}",
     journal   = "Eur. Phys. J.",
     volume    = "A10",
     year      = "2001",
     pages     = "207-215",
     doi       = "10.1007/s100500170132",
     SLACcitation  = "%%CITATION = EPHJA,A10,207;%%"
}
@Article{Leukel:2001,
     author    = "Leukel, Roman",
     journal   = "PhD thesis, Mainz (2001),  http://wwwa2.kph.uni-maiz.de/A2/",
     year      = "2009"
}
@Article{Preobrajenski:2001,
     author    = "Preobrajenski,Ilia",
     journal   = "PhD thesis, Mainz (2001),  http://wwwa2.kph.uni-maiz.de/A2/",
     year      = "2009"
}
@Article{Wolf:2001ha,
     author    = "Wolf, S. and others",
     title     = "{Compton scattering by the proton using a large-acceptance
                  arrangement}",
     journal   = "Eur. Phys. J.",
     volume    = "A12",
     year      = "2001",
     pages     = "231-252",
     eprint    = "nucl-ex/0109013",
     archivePrefix = "arXiv",
     doi       = "10.1007/s100500170031",
     SLACcitation  = "%%CITATION = NUCL-EX/0109013;%%"
}
@Article{Fearing:2000uy,
     author    = "Fearing, Harold W. and Hemmert, Thomas R. and Lewis, Randy
                  and Unkmeir, Christine",
     title     = "{Radiative pion capture by a nucleon}",
     journal   = "Phys. Rev.",
     volume    = "C62",
     year      = "2000",
     pages     = "054006",
     eprint    = "hep-ph/0005213",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.62.054006",
     SLACcitation  = "%%CITATION = HEP-PH/0005213;%%"
}
@Article{Bernard:1994gm,
     author    = "Bernard, V. and Kaiser, Norbert and Meissner, Ulf-G.",
     title     = "{Neutral pion photoproduction off nucleons revisited}",
     journal   = "Z. Phys.",
     volume    = "C70",
     year      = "1996",
     pages     = "483-498",
     eprint    = "hep-ph/9411287",
     archivePrefix = "arXiv",
     doi       = "10.1007/s002880050126",
     SLACcitation  = "%%CITATION = HEP-PH/9411287;%%"
}
@Article{Pfeil:1974ib,
     author    = "Pfeil, W. and Rollnik, H. and Stankowski, S.",
     title     = "{A partial-wave analysis for proton Compton scattering in
                  the delta(1232) energy region}",
     journal   = "Nucl. Phys.",
     volume    = "B73",
     year      = "1974",
     pages     = "166-188",
     doi       = "10.1016/0550-3213(74)90047-9",
     SLACcitation  = "%%CITATION = NUPHA,B73,166;%%"
}
@Article{Arndt:1989ww,
     author    = "Arndt, Richard A. and Workman, Ron L. and Li, Zhujun and
                  Roper, L. David",
     title     = "{Partial wave analysis of pion photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "C42",
     year      = "1990",
     pages     = "1853-1863",
     doi       = "10.1103/PhysRevC.42.1853",
     SLACcitation  = "%%CITATION = PHRVA,C42,1853;%%"
}
@Article{Watson:1954uc,
     author    = "Watson, Kenneth M.",
     title     = "{Some general relations between the photoproduction and
                  scattering of pi mesons}",
     journal   = "Phys. Rev.",
     volume    = "95",
     year      = "1954",
     pages     = "228-236",
     doi       = "10.1103/PhysRev.95.228",
     SLACcitation  = "%%CITATION = PHRVA,95,228;%%"
}
@Article{Shafi:2004zn,
     author    = "Shafi, A. and others",
 collaboration = "Crystal Ball",
     title     = "{Measurement of inverse pion photoproduction at energies
                  spanning the  N(1440) resonance}",
     journal   = "Phys. Rev.",
     volume    = "C70",
     year      = "2004",
     pages     = "035204",
     eprint    = "nucl-ex/0405026",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.70.035204",
     SLACcitation  = "%%CITATION = NUCL-EX/0405026;%%"
}
@Article{Rentmeester:2003mf,
     author    = "Rentmeester, M. C. M. and Timmermans, R. G. E. and de
                  Swart, J. J.",
     title     = "{Determination of the chiral coupling constants c(3) and
                  c(4) in new p p  and n p partial-wave analyses}",
     journal   = "Phys. Rev.",
     volume    = "C67",
     year      = "2003",
     pages     = "044001",
     eprint    = "nucl-th/0302080",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.67.044001",
     SLACcitation  = "%%CITATION = NUCL-TH/0302080;%%"
}
@Article{Buettiker:1999ap,
     author    = "Buettiker, Paul and Meissner, Ulf-G.",
     title     = "{Pion nucleon scattering inside the Mandelstam triangle}",
     journal   = "Nucl. Phys.",
     volume    = "A668",
     year      = "2000",
     pages     = "97-112",
     eprint    = "hep-ph/9908247",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(99)00813-1",
     SLACcitation  = "%%CITATION = HEP-PH/9908247;%%"
}
@Article{Krebs:2007rh,
     author    = "Krebs, Hermann and Epelbaum, Evgeny and Meissner, Ulf-G.",
     title     = "{Nuclear forces with Delta-excitations up to next-to-next-
                  to-leading order I: peripheral nucleon-nucleon waves}",
     journal   = "Eur. Phys. J.",
     volume    = "A32",
     year      = "2007",
     pages     = "127-137",
     eprint    = "nucl-th/0703087",
     archivePrefix = "arXiv",
     doi       = "10.1140/epja/i2007-10372-y",
     SLACcitation  = "%%CITATION = NUCL-TH/0703087;%%"
}

@Article{Timmermans:1990tz,
     author    = "Timmermans, R. G. E. and Rijken, T. A. and de Swart, J. J.
                  ",
     title     = "{Determination of the charged pion coupling constant from
                  data on the charge exchange reaction anti-p p $\to$ anti-n
                  n}",
     journal   = "Phys. Rev. Lett.",
     volume    = "67",
     year      = "1991",
     pages     = "1074-1077",
     doi       = "10.1103/PhysRevLett.67.1074",
     SLACcitation  = "%%CITATION = PRLTA,67,1074;%%"
}


@Article{Fettes:2000xg,
     author    = "Fettes, Nadia and Meissner, Ulf-G.",
     title     = "{Pion nucleon scattering in chiral perturbation theory. II:
                  Fourth order  calculation}",
     journal   = "Nucl. Phys.",
     volume    = "A676",
     year      = "2000",
     pages     = "311",
     eprint    = "hep-ph/0002162",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(00)00199-8",
     SLACcitation  = "%%CITATION = HEP-PH/0002162;%%"
}
@Article{Meissner:2005ne,
     author    = "Meissner, Ulf-G. and Raha, Udit and Rusetsky, Akaki",
     title     = "{Isospin-breaking corrections in the pion deuteron
                  scattering length}",
     journal   = "Phys. Lett.",
     volume    = "B639",
     year      = "2006",
     pages     = "478-482",
     eprint    = "nucl-th/0512035",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.physletb.2006.07.001",
     SLACcitation  = "%%CITATION = NUCL-TH/0512035;%%"
}
@Article{Bernard:1996gq,
     author    = "Bernard, V. and Kaiser, Norbert and Meissner, Ulf-G.",
     title     = "{Determination of the low-energy constants of the next-to-
                  leading order  chiral pion nucleon Lagrangian}",
     journal   = "Nucl. Phys.",
     volume    = "A615",
     year      = "1997",
     pages     = "483-500",
     eprint    = "hep-ph/9611253",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(97)00021-3",
     SLACcitation  = "%%CITATION = HEP-PH/9611253;%%"
}
@Article{Matsinos:1997pb,
     author    = "Matsinos, E.",
     title     = "{Isospin violation in the pi N system at low energies}",
     journal   = "Phys. Rev.",
     volume    = "C56",
     year      = "1997",
     pages     = "3014-3025",
     doi       = "10.1103/PhysRevC.56.3014",
     SLACcitation  = "%%CITATION = PHRVA,C56,3014;%%"
}
@Article{Meissner:1999vr,
     author    = "Meissner, Ulf-G. and Oller, J. A.",
     title     = "{Chiral unitary meson baryon dynamics in the presence of
                  resonances:  Elastic pion nucleon scattering}",
     journal   = "Nucl. Phys.",
     volume    = "A673",
     year      = "2000",
     pages     = "311-334",
     eprint    = "nucl-th/9912026",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(00)00150-0",
     SLACcitation  = "%%CITATION = NUCL-TH/9912026;%%"
}
@Article{Stingl:1974im,
     author    = "Stingl, M. and Rinat, A. S.",
     title     = "{Partial Wave Dispersion Relations for the Nonrelativistic
                  Five Nucleon System}",
     journal   = "Phys. Rev.",
     volume    = "C10",
     year      = "1974",
     pages     = "1253",
     doi       = "10.1103/PhysRevC.10.1253",
     SLACcitation  = "%%CITATION = PHRVA,C10,1253;%%"
}
@Article{1971AnPhy..65..141R,
   author = {{Rinat (Reiner)}, A.~S. and {Stingl}, M.},
    title = "{Multichannel N/D approach to nuclear reactions amongst light nuclei. I. General theory}",
  journal = {Annals of Physics},
     year = 1971,
   volume = 65,
    pages = {141-180},
      doi = {10.1016/0003-4916(71)90165-5},
   adsurl = {http://adsabs.harvard.edu/abs/1971AnPhy..65..141R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@Article{PhysRev.126.1596,
  title = {Singularities in Partial-Wave Amplitudes for Two Ingoing and Two Outgoing Particles},
  author = {Kennedy, J.  and Spearman, T. D.},
  journal = {Phys. Rev.},
  volume = {126},
  number = {4},
  pages = {1596--1602},
  numpages = {6},
  year = {1962},
  month = {May},
  doi = {10.1103/PhysRev.126.1596},
  publisher = {American Physical Society}
}
@Article{Kamalov:2001qg,
     author    = "Kamalov, S. S. and Chen, Guan-Yeu and Yang, Shin-Nan and
                  Drechsel, D. and Tiator, L.",
     title     = "{pi0 photo- and electroproduction at threshold within a
                  dynamical model}",
     journal   = "Phys. Lett.",
     volume    = "B522",
     year      = "2001",
     pages     = "27-36",
     eprint    = "nucl-th/0107017",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-2693(01)01241-2",
     SLACcitation  = "%%CITATION = NUCL-TH/0107017;%%"
}
@Article{Pearce:1989re,
     author    = "Pearce, B. C. and Afnan, I. R.",
     title     = "{THREE-BODY UNITARITY, THE CLOUDY BAG MODEL AND THE ROPER
                  RESONANCE}",
     journal   = "Phys. Rev.",
     volume    = "C40",
     year      = "1989",
     pages     = "220-236",
     doi       = "10.1103/PhysRevC.40.220",
     SLACcitation  = "%%CITATION = PHRVA,C40,220;%%"
}
@Article{Lensky:2009uv,
     author    = "Lensky, Vadim and Pascalutsa, Vladimir",
     title     = "{Predictive powers of chiral perturbation theory in Compton
                  scattering off protons}",
     journal   = "Eur. Phys. J.",
     volume    = "C65",
     year      = "2010",
     pages     = "195-209",
     eprint    = "0907.0451",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1140/epjc/s10052-009-1183-z",
     SLACcitation  = "%%CITATION = 0907.0451;%%"
}
@Article{Baru:2010xn,
     author    = "Baru, V. and others",
     title     = "{Precision calculation of the $\pi^-$ deuteron scattering
                  length and its impact on threshold pi-N scattering}",
     year      = "2010",
     eprint    = "1003.4444",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     SLACcitation  = "%%CITATION = 1003.4444;%%"
}
@Article{vanAntwerpen:1994vh,
     author    = "van Antwerpen, C. H. M. and Afnan, I. R.",
     title     = "{A Gauge invariant unitary theory for pion
                  photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "C52",
     year      = "1995",
     pages     = "554-567",
     eprint    = "nucl-th/9407038",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.52.554",
     SLACcitation  = "%%CITATION = NUCL-TH/9407038;%%"
}
@Article{GomezNicola:1999pu,
     author    = "Gomez Nicola, A. and Pelaez, J. R.",
     title     = "{Unitarized pion nucleon scattering within heavy baryon
                  chiral  perturbation theory}",
     journal   = "Phys. Rev.",
     volume    = "D62",
     year      = "2000",
     pages     = "017502",
     eprint    = "hep-ph/9912512",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevD.62.017502",
     SLACcitation  = "%%CITATION = HEP-PH/9912512;%%"
}
@Article{GomezNicola:2000wk,
     author    = "Gomez Nicola, A. and Nieves, J. and Pelaez, J. R. and Ruiz
                  Arriola, E.",
     title     = "{Improved unitarized heavy baryon chiral perturbation
                  theory for pi N  scattering}",
     journal   = "Phys. Lett.",
     volume    = "B486",
     year      = "2000",
     pages     = "77-85",
     eprint    = "hep-ph/0006043",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-2693(00)00761-9",
     SLACcitation  = "%%CITATION = HEP-PH/0006043;%%"
}
@Article{Nicola:2003zi,
     author    = "Nicola, A. Gomez and Nieves, J. and Pelaez, J. R. and
                  Arriola, E. Ruiz",
     title     = "{Improved unitarized heavy baryon chiral perturbation
                  theory for pi N  scattering to fourth order}",
     journal   = "Phys. Rev.",
     volume    = "D69",
     year      = "2004",
     pages     = "076007",
     eprint    = "nucl-th/0312034",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevD.69.076007",
     SLACcitation  = "%%CITATION = NUCL-TH/0312034;%%"
}
@Article{FernandezRamirez:2009jb,
     author    = "Fernandez-Ramirez, C. and Bernstein, A. M. and Donnelly, T.
                  W.",
     title     = "{The unexpected impact of D waves in low-energy neutral
                  pion photoproduction from the proton and the extraction of
                  multipoles}",
     journal   = "Phys. Rev.",
     volume    = "C80",
     year      = "2009",
     pages     = "065201",
     eprint    = "0907.3463",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1103/PhysRevC.80.065201",
     SLACcitation  = "%%CITATION = 0907.3463;%%"
}

@Article{Ahrens:2001qt,
     author    = "Ahrens, J. and others",
 collaboration = "GDH",
     title     = "{First measurement of the Gerasimov-Drell-Hearn integral
                  for Hydrogen from 200 to 800 MeV}",
     journal   = "Phys. Rev. Lett.",
     volume    = "87",
     year      = "2001",
     pages     = "022003",
     eprint    = "hep-ex/0105089",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevLett.87.022003",
     SLACcitation  = "%%CITATION = HEP-EX/0105089;%%"
}
@Article{Dutz:2003mm,
     author    = "Dutz, H. and others",
 collaboration = "GDH",
     title     = "{First measurement of the Gerasimov-Drell-Hearn sum rule
                  for H-1 from 0.7-GeV to 1.8-GeV at ELSA}",
     journal   = "Phys. Rev. Lett.",
     volume    = "91",
     year      = "2003",
     pages     = "192001",
     doi       = "10.1103/PhysRevLett.91.192001",
     SLACcitation  = "%%CITATION = PRLTA,91,192001;%%"
}
@Article{Holstein:1999uu,
     author    = "Holstein, Barry R. and Drechsel, D. and Pasquini, B. and
                  Vanderhaeghen, M.",
     title     = "{Higher order polarizabilities of the proton}",
     journal   = "Phys. Rev.",
     volume    = "C61",
     year      = "2000",
     pages     = "034316",
     eprint    = "hep-ph/9910427",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.61.034316",
     SLACcitation  = "%%CITATION = HEP-PH/9910427;%%"
}
@Article{Gellas:2000mx,
     author    = "Gellas, George C. and Hemmert, Thomas R. and Meissner,
                  Ulf-G.",
     title     = "{Complete one-loop analysis of the nucleon's spin
                  polarizabilities}",
     journal   = "Phys. Rev. Lett.",
     volume    = "85",
     year      = "2000",
     pages     = "14-17",
     eprint    = "nucl-th/0002027",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevLett.85.14",
     SLACcitation  = "%%CITATION = NUCL-TH/0002027;%%"
}
@Article{Gellas:2001yv,
     author    = "Gellas, G. C. and Hemmert, T. R. and Meissner, U. G.",
     title     = "{Gellas, Hemmert, and Meissner reply to Comment on
                  'Complete one-loop analysis of the nucleon's spin
                  polarizabilities'}",
     journal   = "Phys. Rev. Lett.",
     volume    = "86",
     year      = "2001",
     pages     = "3205",
     doi       = "10.1103/PhysRevLett.86.3205",
     SLACcitation  = "%%CITATION = PRLTA,86,3205;%%"
}
@Article{VijayaKumar:2000pv,
     author    = "Vijaya Kumar, K. B. and McGovern, Judith A. and Birse,
                  Michael C.",
     title     = "{Spin polarisabilities of the nucleon at NLO in the chiral
                  expansion}",
     journal   = "Phys. Lett.",
     volume    = "B479",
     year      = "2000",
     pages     = "167-172",
     eprint    = "hep-ph/0002133",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-2693(00)00340-3",
     SLACcitation  = "%%CITATION = HEP-PH/0002133;%%"
}
@Article{Drechsel:2002ar,
     author    = "Drechsel, D. and Pasquini, B. and Vanderhaeghen, M.",
     title     = "{Dispersion relations in real and virtual Compton
                  scattering}",
     journal   = "Phys. Rept.",
     volume    = "378",
     year      = "2003",
     pages     = "99-205",
     eprint    = "hep-ph/0212124",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0370-1573(02)00636-1",
     SLACcitation  = "%%CITATION = HEP-PH/0212124;%%"
}
@Article{Pasquini:2007hf,
     author    = "Pasquini, B. and Drechsel, D. and Vanderhaeghen, M.",
     title     = "{Proton spin polarizabilities from polarized Compton
                  scattering}",
     journal   = "Phys. Rev.",
     volume    = "C76",
     year      = "2007",
     pages     = "015203",
     eprint    = "0705.0282",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1103/PhysRevC.76.015203",
     SLACcitation  = "%%CITATION = 0705.0282;%%"
}

@Article{Danilkin:2010xd,
     author    = "Danilkin, I. V. and Gasparyan, A. M. and Lutz, M. F. M.",
     title     = "{On causality, unitarity and perturbative expansions}",
     journal   = "Phys. Lett.",
     volume    = "in print",
     year      = "2010",
     eprint    = "1009.5928",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     SLACcitation  = "%%CITATION = 1009.5928;%%"
}

@Article{Gasparyan:2010fb,
     author    = "Gasparyan, A. M. and Lutz, M. F. M.",
     title     = "{Spin observables in pion photoproduction from a unitary
                  and causal effective field theory}",
     year      = "1999",
     eprint    = "9904290",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     SLACcitation  = "%%CITATION = PHRVA,C61,015204;%%"
}
@Article{Drechsel:1999rf,
     author    = "Drechsel, D. and Gorchtein, M. and Pasquini, B. and
                  Vanderhaeghen, M.",
     title     = "{Fixed-t subtracted dispersion relations for Compton
                  scattering off the  nucleon}",
     journal   = "Phys. Rev.",
     volume    = "C61",
     year      = "1999",
     pages     = "015204",
     eprint    = "hep-ph/9904290",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.61.015204",
     SLACcitation  = "%%CITATION = HEP-PH/9904290;%%"
}
@Article{Hildebrandt:2003fm,
     author    = "Hildebrandt, Robert P. and Griesshammer, Harald W. and
                  Hemmert, Thomas R. and Pasquini, Barbara",
     title     = "{Signatures of chiral dynamics in low energy Compton
                  scattering off the  nucleon}",
     journal   = "Eur. Phys. J.",
     volume    = "A20",
     year      = "2004",
     pages     = "293-315",
     eprint    = "nucl-th/0307070",
     archivePrefix = "arXiv",
     doi       = "10.1140/epja/i2003-10144-9",
     SLACcitation  = "%%CITATION = NUCL-TH/0307070;%%"
}
@Article{Hildebrandt:2003md,
     author    = "Hildebrandt, Robert P. and Griesshammer, Harald W. and
                  Hemmert, Thomas R.",
     title     = "{Spin polarizabilities of the nucleon from polarized low
                  energy Compton  scattering}",
     journal   = "Eur. Phys. J.",
     volume    = "A20",
     year      = "2004",
     pages     = "329-344",
     eprint    = "nucl-th/0308054",
     archivePrefix = "arXiv",
     doi       = "10.1140/epja/i2003-10164-5",
     SLACcitation  = "%%CITATION = NUCL-TH/0308054;%%"
}
@Article{Pasquini:2010zr,
     author    = "Pasquini, B. and Pedroni, P. and Drechsel, D.",
     title     = "{Higher order forward spin polarizability}",
     journal   = "Phys. Lett.",
     volume    = "B687",
     year      = "2010",
     pages     = "160-166",
     eprint    = "1001.4230",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1016/j.physletb.2010.03.007",
     SLACcitation  = "%%CITATION = 1001.4230;%%"
}


@Article{PhysRevD.48.1225,
  title = {Helicity-coupling amplitudes in tensor formalism},
  author = {Chung, S. U.},
  journal = {Phys. Rev. D},
  volume = {48},
  number = {3},
  pages = {1225--1239},
  numpages = {14},
  year = {1993},
  month = {Aug},
  doi = {10.1103/PhysRevD.48.1225},
  publisher = {American Physical Society}
}

@Article{Chung:2007nn,
     author    = "Chung, Suh-Urk and Friedrich, Jan",
     title     = "{Covariant Helicity-Coupling Amplitudes: A New
                  Formulation}",
     journal   = "Phys. Rev.",
     volume    = "D78",
     year      = "2008",
     pages     = "074027",
     eprint    = "0711.3143",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1103/PhysRevD.78.074027",
     SLACcitation  = "%%CITATION = 0711.3143;%%"
}

